"The teachers are confused as well": A Multiple-Stakeholder Ethics Discussion on Large Language Models in Computing Education

Large Language Models (LLMs) are advancing quickly and impacting people's lives for better or worse. In higher education, concerns have emerged such as students' misuse of LLMs and degraded education outcomes. To unpack the ethical concerns of LLMs for higher education, we conducted a case study consisting of stakeholder interviews (n=20) in higher education computer science. We found that students use several distinct mental models to interact with LLMs - LLMs serve as a tool for (a) writing, (b) coding, and (c) information retrieval, which differ somewhat in ethical considerations. Students and teachers brought up ethical issues that directly impact them, such as inaccurate LLM responses, hallucinations, biases, privacy leakage, and academic integrity issues. Participants emphasized the necessity of guidance and rules for the use of LLMs in higher education, including teaching digital literacy, rethinking education, and having cautious and contextual policies. We reflect on the ethical challenges and propose solutions.

==> dumped_results.tex <==
\subsection{Diverse Use Cases}
A few people used ChatGPT relatively less. D1 was originally from China and came to the US only recently. He attributed his infrequent use to Internet censorship in China, \textit{``I can’t use ChatGPT in China, so I don’t use it much now.''} P1 had not found many use cases of ChatGPT by the time of the study, but said she would use it ``a bit more in the future.'' Other participants used ChatGPT regularly.

\noindent \textbf{Q\&A.} ChatGPT was used for Q\&A by three industrial professionals and 8 out of 12 students at different levels. Learning scenarios ranged from Japanese (D2) to robotics (M2). I3 asked ChatGPT about technical concepts and treated it as a learning tool. M3 inquired ChatGPT about the parts of academic papers or course slides that she did not understand. U4 used ChatGPT to ``understand things'', from research papers to programming concepts (e.g., data structures, stack), and have more information before going to TA office hours. Three participants compared ChatGPT to search engines and thought it was better in terms of providing more domain-specific information, e.g., ``Better version of Google when I don't know a term'' (I1). M4 further suggested ChatGPT outperformed Wikipedia by generating concise responses, \textit{``When you’re extremely interested in learning something overnight, you
don’t need to look at many pages [in Wikipedia].''} As we can see, ChatGPT's Q\&A capability strikes a balance between informativeness and conciseness. 

\noindent \textbf{Writing Code, Debugging, and Comment Generation.} 
Five students, two professors, and two industrial practitioners used ChatGPT to directly generate code or algorithms, which saved time and improved efficiency for them. For instance, M4 utilized ChatGPT to write Python and SQL code and conduct data processing, which in his eyes was dirty work, \textit{``You know how to write it [code]. It just takes time for you to write it. Data processing is also dirty work, just transforming data from one form to another.''}	Powered by ChatGPT, he was able to simultaneously work on 3-4 projects, but he thought carefully about questions, i.e., ``reshaping or tweaking the question, code, data structure, and data at hand'' to avoid leakage of user data during his internship as a data engineer. 
% He also leveraged ChatGPT to build a smart home system. Implementing the programs by himself, otherwise, would ``take a lot of life experience and time.'' 
U2 generated Python code with ChatGPT when she did not know how to get started. She used it as a hint, a template, and a reference, and did not think there was an authorship concern, \textit{``Essays have authorship concerns. Algorithms are the same, just different variables.''} 

Most of the participants acknowledged that ChatGPT-generated code was not perfect, especially for complicated tasks, but provided insights for their own coding. They always applied error checking and modification, even for simple, common code, which ChatGPT was relatively good at generating. I1 suggested that ChatGPT generation was based on probability instead of logic, making its code more likely to contain errors.
% \textit{``I use ChatGPT to write common code. I think it’s better than me, but I’ll double-check to make sure I understand the code. I do error-checking because I'm not that confident about the results. ChatGPT is a likelihood-based model, not necessarily understanding the logic.''} 
% He relied on ChatGPT more for insights and frameworks, e.g., how people use a certain package, what a parameter means, and what a good design structure looks like, \textit{``It gives directions even if the code does not work.''}
M3 similarly articulated that ChatGPT could not find good solutions to coding problems and mostly used its code to understand other programmers’ perspectives. P2, a professor, used ChatGPT API to extract sentences with certain biomedical terms from academic articles, reaching an accuracy of 40\%, which was not as good as fine-tuned BERT. I4, an industrial ML engineer, used ChatGPT API to generate labels for news articles on the platform he built. He combined prompt engineering and human work to eliminate errors produced by ChatGPT, \textit{``
% I can’t guarantee the reliability of ChatGPT output, but it's much better than other open-source models. 
We would remove redundant output such as `I’m an OpenAI model' by specifying the requirement and asking it to generate again. If errors happen three times, human work will intervene.''} The participants who did not use ChatGPT for coding-related tasks thought coding was too complicated for ChatGPT (U1), were afraid of violating no-ChatGPT policy in courses (U4), and thought specifying coding requirements for ChatGPT was time-consuming (M2).

Three participants debugged or optimized their code using ChatGPT. M2 said sometimes ChatGPT successfully figured out errors in her code and gave her a high-level understanding, but she had to correct errors manually. U4 used ChatGPT to debug code in hard CS courses. He estimated that ChatGPT identified bugs 6 out of 10 times; in other cases, ChatGPT returned the same code as his own. I3 expressed that using ChatGPT to optimize code was overall helpful as long as a human was in the loop since it may make up libraries.

Two industrial practitioners, whose jobs required generating high-quality comments for code, used ChatGPT to assist with this task. I4 thought comment generation was made easier by collaborating with ChatGPT and the comments were more readable for other team members. Comment generation required heavy manual work and memorization of code details. ChatGPT helped I1 with these headaches, \textit{``Code comments are a lot of manual work. I'm lazy and I don’t like typing comments. Also, after weeks, I don’t know what the code is doing. ChatGPT is useful, saving me a lot of time.''}

% U4 was told by the instructors not to use ChatGPT to generate code, both through the syllabus and verbally, \textit{``TAs mentioned anti-cheating programs. I didn’t try that [generating code with ChatGPT], but some students did it.''} 
% Some only asked ChatGPT to generate a  high-level framework for code. M2 was such a case. She thought telling ChatGPT detailed requirements was time-consuming, and she could write code more quickly by herself.

\noindent \textbf{Cautious Use in Assignments.}
Most student participants did not use ChatGPT for assignments. M4 gave his reasons, i.e., professors' rules or caution against ChatGPT use for assignments and willingness to learn, which were representative among other participants as well.
% \textit{``I try to avoid using it [ChatGPT] for assignments except the dumb sides, such as generating SQL code. Some professors think it’s against academic integrity. The courses are good and I want to learn something from them.''} 
When D3 was asked if she used ChatGPT for her assignments, her reaction was: \textit{``It’s not ethical, right?''}

The three students who did use ChatGPT for assignments also took caution during the use. For example, U4 would ask his own questions instead of copying and pasting questions directly from the assignments. Among the five courses he currently took, two professors were against ChatGPT use, and one professor asked students to state ChatGPT prompts they used for the assignments. D1
thought	ChatGPT was not good at hard, theoretical algorithms and only gave
a fundamental answer for his assignment questions, thus he always needed to check its correctness. The syllabus for the course he took also stated that students could not use ChatGPT responses directly, but should use their own words. D3 differentiated between ethical and unethical use of ChatGPT based on whether students applied their thinking to their assignments.
% \textit{``ChatGPT helps me integrate all the results from the search engine. If you use ChatGPT without thinking, it will be unethical. If you know if the answer is wrong or not, it’s fine.''}
She simultaneously expressed the concern that ChatGPT tended to generate similar answers for different students, especially in writing structures, making ChatGPT-generated assignment responses easily identifiable by instructors.

\noindent \textbf{Essay Writing and Research.}
Several students (N=3) did not use ChatGPT for essay writing in courses at all, mainly due to its obvious AI-styled language use and the possibility of being caught by the instructors. U1 was an example. He said, \textit{``I'm not confident if its answers are correct if I use it for writing an essay. The writing is clearly AI-generated. I'm worried about being found by the instructor.''} U3 similarly expressed that ChatGPT-generated essays looked too redundant, formal, and machine-like. M2 planned to write essays with ChatGPT in the future but thought the bottom line was to use her own ideas. 
% Again, she acknowledged that changing the writing styles and fixing details were necessary. 
I2 said, \textit{``I paid a lot for the degree, so I wanted to learn.'' }
One professor, P1, did not use ChatGPT for writing academic papers since she did not know how to disclose its use in research. Thus, she felt writing papers with ChatGPT was ``not the right thing to do.''

For those who did use ChatGPT during the essay or paper writing processes, various uses were brought up. Seven participants directly asked ChatGPT to generate content for them. D3 described this ChatGPT-assisted writing process, \textit{``I used ChatGPT for introduction writing. ChatGPT writes better than me. I give it specific instructions like titles and key information. After it generates content, I point out unsatisfactory places and ask it to revise.''} ChatGPT often came to the rescue when people felt difficulty generating content by themselves. M3 used ChatGPT whenever she could not convey thoughts by herself when writing an essay in a research-oriented NLP course. 
% She recalled that the instructor did not have any restrictions on LLM use and said ideas were the most important thing. 
She was satisfied with the writing of ChatGPT, rating it 8 out of 10. P3 used ChatGPT in a similar manner, i.e., asking it to generate a paragraph when stuck, \textit{``At least I get a thing to get started. I'm no longer on an empty page.''} 
% P2 was yet another example, \textit{``ChatGPT has a basic output and I change a lot of it, adding my personal style. It prevents me from starting from an empty page.''}
Some were more cautious when using ChatGPT to generate content. For instance, I3 only used ChatGPT to generate catchy titles, not paragraphs, \textit{``We write things in a certain way. I want to make it consistent.''} 
% U2 was concerned about ChatGPT-style essays which contained redundant paragraphs. She thought instructors had some ways to identify ChatGPT-generated essays and would only borrow ideas from ChatGPT-generated content. She also thought directly using ChatGPT-generated essays was not fair to other students who wrote essays with their efforts.

Seven participants used ChatGPT to polish up their writing or conduct a grammar and typo check. P2 acknowledged that as a non-native speaker, the transition between paragraphs and subtle expressions was hard, whereas ChatGPT showed a better understanding. I1 usually had a first draft and then combined it with the revised version output by ChatGPT. As a proofreader, ChatGPT was not perfect. U2 noted that ChatGPT tended to oversimplify statements and refused to use ``fancy words.'' D4 mentioned repeated patterns in the essays after ChatGPT's revision. He only used some parts of the refining to avoid his essays from being recognized as AI-generated.

Another common use of ChatGPT in writing was ideation and brainstorming (N=7). M1 once asked ChatGPT to generate 20 potential ideas for his course project, from which he chose one with his thinking. The instructor researched generative AI and creativity, so she encouraged students to use ChatGPT and did not enforce any policies against its use. I3 recalled a scenario where ChatGPT reminded her of missing points during the ideation phase of a research paper, which she verified and adopted with caution, \textit{``I was writing an article on healthcare and generative AI. I gave ChatGPT an outline, asking, `Am I missing anything?' It suggested mental health as an additional topic and relevant products. I was not sure if it was a hallucination. It's a futurist, so the products will probably come soon. It gives me thinking anyway.''} D3 treated ChatGPT as a search engine to quickly learn a field, which helped her generate ideas. She did not think ChatGPT, which ``had no judgment,'' could generate research ideas, which ``required critical and detailed thinking.''  

Three participants used ChatGPT to help with the literature review process. U2 asked ChatGPT to suggest references, which she thought had nothing to do with original ideas. In pre-ChatGPT times, she sometimes spent 3-4 hours manually searching papers without finding anything. ChatGPT boosted her efficiency in gathering the related work. D2 heavily drew on ChatGPT in producing an annotated bibliography. P4 would ask ChatGPT to give him an overview of a certain topic and use it as a starting point for literature review. I2 did not feel like reading an 80-page paper and asked Bing Chat to summarize it for her.

% P3 did not employ ChatGPT in the literature review process for concerns of hallucination.

\noindent \textbf{Teaching.}
Only one out of four professors indicated using ChatGPT in the teaching process. P2 used ChatGPT to generate a syllabus for a course on LLMs, though he changed it a lot. He thought ChatGPT was helpful in this process. He also mentioned that ChatGPT was good at explaining concepts in a novice way and giving analogies, which he used in class on a few occasions. P3, on the contrary, did not use ChatGPT for teaching as she was skeptical and nervous that ChatGPT-generated content was not always right. In addition, she often taught familiar courses and did not see a need to overhaul the syllabus and teaching materials. Similarly, P4 did not use ChatGPT for teaching since ``previous instructors had pretty detailed teaching materials and the auto-grading system for code assignments and multi-choice questions was already implemented.'' D2, who would teach a writing course in the upcoming semester, foresaw several uses of ChatGPT, such as checking grammar issues in the syllabus and assignment requirements and generating ``bad samples'' for students to learn the grading criteria, \textit{``You can’t use students’ essays as bad examples.''} She would not use ChatGPT to grade students' assignments for both privacy and copyright concerns. According to her, students’ consent was required in such cases; however, students' consent was usually ``forced consent'' given the power imbalance between them and instructors.

\noindent \textbf{Non-native Speakers' Use.}
ChatGPT was frequently used by non-native speakers for generating synonyms, writing emails, paraphrasing writing, and learning English. M3 thought ChatGPT's performance in composing emails was fine (9.5/10) since the task did not require strict structures and wording. However, I1 mentioned grammar errors in ChatGPT-generated emails, so he had to manually check its version and further make the emails into his own style. By treating ChatGPT as a robot, M4 felt no shame asking it to polish up his writing, \textit{``No one wants to spend time helping you polish up your writing. ChatGPT is a robot, so you don’t feel shame asking it to help your email. You don’t worry about wasting its time.''} When writing papers, P2 also used ChatGPT to help him find the right words and thus appear more professional. However, D2 cautioned that ChatGPT revision may change meaning. When U2 prepared for the writing portion of the TOEFL test, she asked ChatGPT for perspectives to approach certain topics. She would also ask ChatGPT to generate a formative assessment for her writing sample.



% from zak
% Using ChatGPT to do research, on the other hand, raised fewer academic integrity concerns than students' cheating. It was agreed that ideas were the most important thing in research, which ChatGPT was not good at. D3 articulated that ChatGPT would ``only generate general answers utilizing average human intelligence as a probability model and couldn't generate good research ideas.'' I2, however, was worried about collaborators' use of ChatGPT in writing papers as she could tell the nuances in ChatGPT-generated content.

% \textbf{Human Autonomy}

% \zakcomment{I think this whole section should be taken out. Human autonomy is different than this discussion - it concerns the ability to act based on your own choices. This discussion is all about anxiety of being replaced by AI in the job market. IMO that's beyond the scope of this paper. However, some of the commented out portions here are usable elsewhere. For example, people talk about the need to co-work with ChatGPT because it can't write an entire project's code (only specific functions), and people are needed to knit together components and run tests, define optimization strategies, etc.}

% Ten participants were optimistic about their career prospects and did not think ChatGPT could replace them. M4 thought ChatGPT was not better than humans but only memorized things better and compared ChatGPT to dictionaries. U3 did not think ChatGPT could write code for entire projects, but just separate functions -- only software engineers were able to knit different components together, e.g., connecting the database and the operating system. ChatGPT was not able to generate test cases and optimization strategies either. Further, ChatGPT could not do user research for designers but only generate wireframes.

% According to D3, ChatGPT lacked critical thinking skills and had no deep understanding of a specific problem. 
% U2 found ChatGPT lacked communication and networking skills which were needed in a software engineer, \textit{``ChatGPT can't go to meetings.''} P1 was not worried about being replaced as a researcher and thought ChatGPT was only good at writing, which was not the core part of her research, \textit{``The core parts of my research are gathering data and talking to people, like going to board meetings.''} I3 thought instead of replacing her, ChatGPT enhanced her ability. I2 also believed ChatGPT helped reduce her workload. Three participants saw a long-term risk of being replaced by ChatGPT, in other words, they were not worried for now. I4 was an example, \textit{``I'm not going to be replaced in 10 years. AI is somewhere close to the ceiling. It's not as intelligent as smart people.''} 
% P3 did not think she would be replaced in her lifetime, \textit{``Not anywhere near that in my lifetime. ChatGPT can teach, but can it do research?''} M1 thought AI would ultimately replace humans in 200 years, even in creativity-oriented jobs. At the same time, he believed humans could stop this process.

% Nine participants thought repetitive, non-creative jobs were more likely to be taken by ChatGPT. 
% I4 said data analysts’ jobs could partly be done by ChatGPT, which helped ``cut some redundancy in human resources.'' 
% D1 talked about the evolution of jobs, \textit{``In 2010, software development was a creative job, but now it is less innovative.''}
% P2 found ChatGPT better at extracting information from papers, synthesizing literature, and writing, but worse at generating ideas. 
% U4 did not think jobs that required communication skills and critical thinking skills could be taken by AI. 
% U2 thought coding and SDE jobs were likely to be replaced since ChatGPT knew algorithms better than her. She thought SDE jobs would evolve in the future and focus more on making internal infrastructures more secure or other ethical aspects. 
% Thus, she was still capable. 
% M3 explained why creative jobs were less likely to be replaced than repetitive jobs, \textit{``Humans are different than machines and better at ideas. Machines can’t create things, but only follow patterns and combine knowledge.''} 
% M4 cited the quote of James Landay, \textit{``ChatGPT is not innovative. Instead of replacing people with AI, we can augment people with AI and give them more autonomy.''} 
% P4 thought the repetitive part of his research could be done by ChatGPT, e.g., literature review and data labeling, where ChatGPT empowered researchers by freeing them from ``unenjoyable work'' and mitigating inequality between big and small research groups. On the other hand, innovative tasks such as identifying emerging problems in CS, interpreting social aspects of IT, and building information channels could not be done by ChatGPT. P1 argued that we needed to think about what were necessary jobs for people to do and called pencil-pushing and data entry as bullshit jobs.

% P2 expressed concern about getting stupid as a human being, \textit{``
% It's helpful especially if you understand the risks coming with it. Always take it with a grain of salt. When I'm not sure how accurate it is, I will go to Wikipedia for factual information. I ask ChatGPT more for nuanced questions... 
% Will we lose our ability, for example, can't find directions without smartphones? I'm always a little worried about getting stupid.''}




% Thus, student work was less likely to be done by ChatGPT. She was also not worried about ChatGPT-generated code, \textit{``Your friend can also program for you. You’re an adult.''} P2 similarly pointed out that students were more likely to cheat in humanistic courses where writing was the main assessment tool.



% Similarly, M4 worried more about the research subjects' data than his own data. He saw disclosing participant information as a betrayal and used an analogy to illustrate such data leakage, \textit{``It's like my best friend tells me the saddest story, then I tell it to another person.''} 

% U1 did not ask ChatGPT private questions but acknowledged not considering ethical implications before the interview. U2 did not dare to give selfies to LLMs.





% She attributed better ethical performance of ChatGPT partly to its standalone nature; the interaction only included herself and ChatGPT, without other users like on social media.
% M4 did not think students' essays contained much innovation and thus were not targets. He further suggested harvesting student assignments from other websites such as Quizlet was more efficient than from ChatGPT. 
% I1 was originally from China, which in his words was a place with no privacy, \textit{``I'm not worried. I don’t care about my privacy. In China, I don’t have privacy.''} 


% P2 thought ChatGPT was just regenerating the social bias without doing anything else, \textit{``It reflects the training data and how our value systems work.''} 
% D1 elaborated on this opinion, \textit{``Bias comes from historical contexts. For example, gender bias comes from labor division in history, where men were better at physically intensive work.''} 
% I3 regarded bias as a form of disagreement or diverse opinions, which was not necessarily a bad thing unless it was about discriminating against a certain group.

% M2 thought students should learn how to not bias other people. 
% D1 may get angry at biased responses and post a tweet on it, but he did not think he had enough time or money to protect his rights. 


% Six others felt less confident in mitigating the impact of biased responses since the bias was deeply rooted in culture and history.

